Revised Filter Profiles and Zero Points for Broadband Photometry

Estimating accurate bolometric fluxes for stars requires reliable photometry to absolutely flux calibrate the spectra. This is a significant problem for studies of very bright stars, which are generally saturated in modern photometric surveys. Instead we must rely on photometry with less precise calibration. We utilize precisely flux-calibrated spectra to derive improved filter bandpasses and zero points for the most common sources of photometry for bright stars. In total we test 40 different filters in the General Catalog of Photometric Data as well as those from Tycho-2 and Hipparcos. We show that utilizing inaccurate filter profiles from the literature can create significant color terms resulting in fluxes that deviate by >10% from actual values. To remedy this we employ an empirical approach; we iteratively adjust the literature filter profile and zero point, convolve it with catalog spectra, and compare to the corresponding flux from the photometry. We adopt the passband values that produces the best agreement between photometry and spectroscopy and is independent of stellar color. We find that while most zero points change by <5%, a few systems change by 10-15%. Our final profiles and zero points are similar to recent estimates from the literature. Based on determinations of systematic errors in our selected spectroscopic libraries, we estimate that most of our improved zero points are accurate to 0.5-1% or better.

==> setup.tex <==
%% For anyone who downloaded my source file from arxiv:
%% I stole most of this setup.tex from a paper by Peter .K.G. Williams, but I made a bunch of edits to satisfy my own needs. You might check his paper out (http://arxiv.org/abs/1409.4411) for the original source file or contact him if you have any questions, since I don't really understand how some of these things work. 
%One cool thing it does is you can define an object, just that when someone clicks on the pdf it will link to simbad. I could never quite get this to work, probably because you have to get the text exactly right and my motivation for getting it to work was not super high. 


% basic packages
\usepackage{amsmath,amssymb}
\usepackage[breaklinks,colorlinks,urlcolor=blue,citecolor=blue,linkcolor=blue]{hyperref}
\usepackage{epsfig}    
\usepackage{graphicx}    
\usepackage{lineno}
\usepackage{natbib}
\usepackage{bigints}
\usepackage[outdir=./]{epstopdf}


% font stuff
\usepackage[T1]{fontenc}
\pwifjournal\else
  \usepackage{microtype}
\fi


% emulateapj has overly conservative figure widths, I think because some
% people's figures don't have good margins. Override.
\pwifjournal\else
  \makeatletter
  \renewcommand\plotone[1]{%
    \centering \leavevmode \setlength{\plot@width}{0.95\linewidth}
    \includegraphics[width={\eps@scaling\plot@width}]{#1}%
  }%
  \makeatother
\fi


% My amazing object-referencing system!
%
% \MakeObj[shortname]{ident}{url-escaped name}{formal name}
%    defines an object
% \MakeTrunc{ident}{truncname}
%    defines a truncated name for a blended object (e.g. LP 349-25 *AB*)
%
% \obj{ident}:  link using standard/short name
% \objf{ident}: link using formal/full name
% \objt{ident}: link using the truncated name
%
% Links are \object{} commands if in journal mode, links to Simbad otherwise.
%
% Under the hood:
%
% \pkgwobj@c@<ident> turns its argument into an appropriate link for the object
% \pkgwobj@f<ident>  expands into the formal/full name of the object
% \pkgwobj@s<ident>  expands into the standard/short name of the object

\makeatletter

\newcommand\@simpfx{http://simbad.u-strasbg.fr/simbad/sim-id?Ident=}

\newcommand\MakeObj[4][\@empty]{% [shortname]{ident}{url-escaped}{formalname}
  \pwifjournal%
    \expandafter\newcommand\csname pkgwobj@c@#2\endcsname[1]{\protect\object[#4]{##1}}%
  \else%
    \expandafter\newcommand\csname pkgwobj@c@#2\endcsname[1]{\href{\@simpfx #3}{##1}}%
  \fi%
  \expandafter\newcommand\csname pkgwobj@f#2\endcsname{#4}%
  \ifx\@empty#1%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#4}%
  \else%
    \expandafter\newcommand\csname pkgwobj@s#2\endcsname{#1}%
  \fi}%

\newcommand\MakeTrunc[2]{% {ident}{truncname}
  \expandafter\newcommand\csname pkgwobj@t#1\endcsname{#2}}%

\newcommand{\obj}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@s#1\endcsname}%
  \fi}
\newcommand{\objf}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@f#1\endcsname}%
  \fi}
\newcommand{\objt}[1]{%
  \expandafter\ifx\csname pkgwobj@c@#1\endcsname\relax%
    \textbf{[unknown object!]}%
  \else%
    \csname pkgwobj@c@#1\endcsname{\csname pkgwobj@t#1\endcsname}%
  \fi}

\makeatother


% Evil magic to patch natbib to only highlight the year paper refs, not the
% authors too; as seen in ApJ. From
% http://tex.stackexchange.com/questions/23227/.

\pwifjournal\else
  \usepackage{etoolbox}
  \makeatletter
  \patchcmd{\NAT@citex}
    {\@citea\NAT@hyper@{%
       \NAT@nmfmt{\NAT@nm}%
       \hyper@natlinkbreak{\NAT@aysep\NAT@spacechar}{\@citeb\@extra@b@citeb}%
       \NAT@date}}
    {\@citea\NAT@nmfmt{\NAT@nm}%
     \NAT@aysep\NAT@spacechar\NAT@hyper@{\NAT@date}}{}{}
  \patchcmd{\NAT@citex}
    {\@citea\NAT@hyper@{%
       \NAT@nmfmt{\NAT@nm}%
       \hyper@natlinkbreak{\NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi}%
         {\@citeb\@extra@b@citeb}%
       \NAT@date}}
    {\@citea\NAT@nmfmt{\NAT@nm}%
     \NAT@spacechar\NAT@@open\if*#1*\else#1\NAT@spacechar\fi\NAT@hyper@{\NAT@date}}
    {}{}
  \makeatother
\fi


% Object data
\MakeObj{n33370}{NLTT\%2033370}{NLTT~33370\,AB}
\MakeTrunc{n33370}{NLTT~33370}
\MakeObj{tvlm}{TVLM\%20513-46546}{TVLM~513--46546}

% utility

\newcommand{\vdag}{(v)^\dagger}
\newcommand{\oxygen}{O$_2$}
\newcommand{\water}{H$_2$O}
\newcommand{\kepler}{{\it Kepler }}
\newcommand{\logg}{$log~g$ }
\newcommand{\metal}{[M/H]}
\newcommand{\um}{$\mu$m}
\newcommand{\fbol}{$F_{\mathrm{bol}}$}
\newcommand{\rapsq}{$R_{ap}^2$}
\newcommand{\rchisq}{$\chi^2_{\nu}$}
\newcommand{\hipp}{{\it Hipparcos}}


\newcommand\aafd{erg~s$^{-1}$~cm$^{-2}$~\AA$^{-1}$} % "AAngstrom flux density"
\newcommand\apx{\ensuremath{\sim}}
\newcommand\cgsflux{erg~s$^{-1}$~cm$^{-2}$}
\newcommand\cgslum{erg~s$^{-1}$}
\newcommand\chandra{\textit{Chandra}}
\newcommand\citeeg[1]{\citep[\eg,][]{#1}}
\newcommand\cps{ct~s$^{-1}$}
\newcommand\dd{\ensuremath{\text{d}}}
\newcommand\eg{\textit{e.g.}}
\newcommand\etal{\textit{et~al.}}
\newcommand\ewha{\ensuremath{\text{EW}(\ha)}}
\newcommand\fig[1]{Figure~\ref{f.#1}}
\newcommand\ha{{\ensuremath{\text{H}\alpha}}}
\newcommand\I{\mathcal{I}}
\newcommand\ie{\textit{i.e.}}
\newcommand\kms{km~s$^{-1}$}
\newcommand\ls{L$_\odot$}
\newcommand\mj{M$_\text{J}$}
\newcommand\ms{M$_\odot$}
\newcommand\nupk{\ensuremath{\nu_\text{pk}}}
\newcommand\percc{cm$^{-3}$}
\newcommand\rcs{\ensuremath{\chi_r^2}}
\newcommand\rj{R$_\text{J}$}
\newcommand\sect[1]{Section~\ref{s.#1}}
\newcommand\sherpa{\textsf{Sherpa}}
\newcommand\sti{Stokes~$I$}
\newcommand\stiv{Stokes~$I$ and~$V$}
\newcommand\stv{Stokes~$V$}
\newcommand\swift{\textit{Swift}}
\newcommand\tb{\ensuremath{T_\text{b}}}
\newcommand\tbl[1]{Table~\ref{t.#1}}
\newcommand\teff{\ensuremath{T_\text{eff}}}
\newcommand\todo[1]{\textcolor{red}{#1}}
\newcommand\ujy{$\mu$Jy}
\newcommand\ujybm{$\mu$Jy~bm$^{-1}$}
\newcommand\uv{$u$\mbox{-}$v$}
\newcommand\vsi{\ensuremath{v \sin i}}
\newcommand\weff{W$_{\rm{eff}}$}

\newcommand\Lb{\ensuremath{L_\text{bol}}}
\newcommand\Lh{\ensuremath{L_\ha}}
\newcommand\Lr{\ensuremath{L_\text{R}}}
\newcommand\sLr{\ensuremath{L_{\nu,\text{R}}}}
\newcommand\Lu{\ensuremath{L_\text{UVW1}}}
\newcommand\Lx{\ensuremath{L_\text{X}}}
\newcommand\Lxf{\ensuremath{L_{\text{X},f}}}
\newcommand\Lxq{\ensuremath{L_{\text{X},q}}}
\newcommand\lb{\ensuremath{[\Lb]}}
\newcommand\lh{\ensuremath{[\Lh]}}
\newcommand\lr{\ensuremath{[\Lr]}}
\newcommand\slr{\ensuremath{[\sLr]}}
\newcommand\lu{\ensuremath{[\Lu]}}
\newcommand\lx{\ensuremath{[\Lx]}}
\newcommand\lxf{\ensuremath{[\Lxf]}}
\newcommand\lxq{\ensuremath{[\Lxq]}}
\newcommand\lhlb{\ensuremath{[\Lh/\Lb]}}
\newcommand\lrlb{\ensuremath{[\Lr/\Lb]}}
\newcommand\lulb{\ensuremath{[\Lu/\Lb]}}
\newcommand\lxlb{\ensuremath{[\Lx/\Lb]}}
\newcommand\lxflb{\ensuremath{[\Lxf/\Lb]}}
\newcommand\lxqlb{\ensuremath{[\Lxq/\Lb]}}
\newcommand\slrlb{\ensuremath{[\sLr/\Lb]}}
\newcommand\slrlx{\ensuremath{[\sLr/\Lx]}}
\newcommand\slrlxf{\ensuremath{[\sLr/\Lxf]}}
\newcommand\slrlxq{\ensuremath{[\sLr/\Lxq]}}

